From Sparse Dependence to Sparse Attention: Unveiling How Chain-of-Thought Enhances Transformer Sample Efficiency

Chain-of-thought (CoT) significantly enhances the reasoning performance of large language models (LLM). While current theoretical studies often attribute this improvement to increased expressiveness and computational capacity, we argue that expressiveness is not the primary limitation in the LLM regime, as current large models will fail on simple tasks. Using a parity-learning setup, we demonstrate that CoT can substantially improve sample efficiency even when the representation power is sufficient. Specifically, with CoT, a transformer can learn the function within polynomial samples, whereas without CoT, the required sample size is exponential. Additionally, we show that CoT simplifies the learning process by introducing sparse sequential dependencies among input tokens, and leads to a sparse and interpretable attention. We validate our theoretical analysis with both synthetic and real-world experiments, confirming that sparsity in attention layers is a key factor of the improvement induced by CoT.

==> ICLR/Main/1-intro.tex <==
\section{Introduction}
Chain-of-thought (CoT) has proven to be a powerful technique for enhancing reasoning in large language models \cite{wei2022chain, kojima2022large}.  By instructing the model to break complex problems into smaller, manageable steps, CoT facilitates more efficient reasoning and better generalization, particularly in algorithmic and logical tasks \cite{nye2022show, lewkowycz2022solving, wang2023selfconsistency}. 
Building on this, performance can be further improved through multi-step prompting and multi-path sampling techniques \cite{JMLR:v24:22-1144, wang2022rationale, zhou2023leasttomost, zhang2023automatic, fu2023complexitybased}.
% such as incorporating self-consistency checks \cite{JMLR:v24:22-1144, wang2022rationale}, increasing problem difficulty within the chain \cite{zhou2023leasttomost}, and employing complexity-based prompting \cite{zhang2023automatic, fu2023complexitybased}. 

This focus on CoT within in-context learning has since expanded to more structured learning approaches \cite{yao2024tree, besta2024graph}. By adding reasoning examples of CoT style to the instruction-tuning dataset, models enhance their problem-solving abilities more effectively than relying solely on CoT during prompting \cite{zelikman2022star, JMLR:v25:23-0870}. As a result, CoT is now shaping a new paradigm in language model development, marking a shift from simply scaling data \cite{kaplan2020scaling, hoffmann2022an} to focusing on advanced reasoning strategies \cite{lightman2024lets}, which leads to more effective learning outcomes.

% Chain-of-thought (CoT) has emerged as a powerful technique for improving reasoning in large language models \cite{wei2022chain, kojima2022large, nyeshow, lightman2024lets}. By breaking complex problems into smaller steps, CoT enables more efficient reasoning and better generalization, especially in algorithmic and logical tasks. This marks a shift from merely scaling data \cite{kaplan2020scaling, hoffmann2022an} to focusing on reasoning strategies like CoT, which is shaping a new paradigm in language model development \cite{wang2023selfconsistency, JMLR:v25:23-0870, yao2024tree}.

% In parallel, significant efforts have been made to improve in-context learning through CoT prompting \cite{JMLR:v24:22-1144, wang2023towards}. For instance, self-consistency methods \cite{JMLR:v24:22-1144} encourage models to generate multiple reasoning paths and select the most consistent one, improving accuracy on a wide range of tasks. Other strategies, such as breaking down complex tasks into simpler sub-problems, as demonstrated in Least-to-Most prompting \cite{zhou2023leasttomost}, also enhance performance. These techniques highlight that structuring the reasoning process, rather than solely increasing model size, can lead to better learning outcomes.

While CoT’s success is well-established, understanding why it works is still a hotly debated topic \cite{saparov2023language, prystawski2024think}. Recent theoretical studies suggest that CoT enhances a model’s expressiveness, increasing its representational capacity when the sequence is long enough \cite{feng2023towards, li2024chain}. However, expressivity alone does not guarantee success. Large language models often struggle with simple tasks—like counting the number of 'r's in "strawberry"—when not using CoT. Given the increasing model sizes, it seems unlikely that such tasks are inherently inexpressible. This discrepancy calls for a deeper study of generalization, hinting the true power of CoT may lie beyond the expressiveness.

% Classical universal approximation theory suggests that even a two-layer network can approximate any function \cite{cybenko1989approximation, HORNIK1989359}, yet in practice, deep networks are the ones that consistently excel. 

In this paper, we study the benefit of CoT from the sample efficiency perspective.  We provide concrete examples where expressiveness is not the limiting factor; that is, the function can be expressed both with and without CoT by the transformers. 
We demonstrate, both in theory and in practice, that without CoT, the learning requires exponentially more samples comparing to with CoT. 
% In other words, {{\bf CoT improves sample efficiency of transformers}}. 
{Further, we show that CoT sequences introduce sparse sequential dependence,  thereby enhancing the sparsity in the attention layers. We then show that transformers can efficiently optimize and generalize on such sequences}. We summarize our contributions as follows.

% We validate with the experiments in Figure~\ref{fig: motivating example}, where we show that 1-layer transformer can easily overfit a parity function if CoT were not provided. 

% Therefore, this work considers CoT from a generalization perspective. Our study starts from the observation that existing expressivity results only require that the sequence is long enough, missing the condition that CoT should describe intermediate reasoning steps.
% Inspired by this, our analysis shows that a valid CoT sequence introduces sparse sequential dependence to reduce sample complexity, explanining why intermediate steps can help model to learn. 

% \jz{rewrite below.}
% We provide both theoretical and empirical evidences to show that CoT improves sample efficiency as tasks become more challenging. More specifically, we consider $k-$parity learning problem. Without CoT, the amount of data required to learn a harder problem would exponentially grwo in parity $k$ compared to learning with CoT. Our analysis is further validated  with numerical experiments.



% Instead, the key challenge lies in efficiently guiding the model through a structured reasoning process, where CoT plays a crucial role. This indicates that scaling expressiveness alone is insufficient for solving certain algorithmic or logic-based tasks, and CoT's capacity to improve sample efficiency could be the critical factor moving forward.


% Like in the work by \cite{kaplan2020scaling}, where the relationship between model size, data size, and performance is thoroughly examined, we here investigate the complexity scaling law along the dimension of problem hardness. Instead of focusing on data or model scaling, we aim to understand how Chain-of-Thought affects sample complexity as the difficulty of problems increases. Our work shifts the focus from expressiveness and dataset size to the efficiency of reasoning processes when tackling more challenging tasks. By analyzing how CoT reduces the number of samples required for complex problems, we provide insights into how reasoning strategies scale with problem complexity, offering a new perspective on performance improvement for harder tasks.




% \vspace{-0.1in}
\begin{enumerate}[leftmargin=*]
\item %Theoretically, we show that while the parity problem can be expressed by a 1-layer transformer, learning requires exponential to $k$ samples without CoT when the number of parameters is limited (Theorem~\ref{thm:rep} and Theorem~\ref{thm:nocot}). Meanwhile, for CoT data with sparse sequential dependency, a 1-layer transformer can learn the parity function and faithfully represent the sparse dependency in its attention pattern with almost linear samples with respect to $k$ and $n$ (Theorem~\ref{thm:main}).
Theoretically, we show that while the parity problem can be expressed by a 1-layer transformer, learning requires exponentially many samples without CoT when the number of parameters is limited (Theorem~\ref{thm:rep} and ~\ref{thm:nocot}). Meanwhile, for CoT data with sparse sequential dependence, a 1-layer transformer can learn the parity function and faithfully represent the sparse dependence in its attention pattern with almost linear samples with respect to sequence length(Theorem~\ref{thm:main}).
\item Empirically, we verify our analysis that training on parity function with CoT data requires only polynomial samples and will induce sparse and interpretable attention (\Cref{fig: sample complexity with CoT and attention}). We further show that evaluating and training on CoT data will also induce sparser attention on real-world dataset GSM-8k on pretrained language models.
\end{enumerate}


% Without CoT, the model attempts to map inputs directly to outputs in one step, which can be a highly complex function to approximate, especially for tasks requiring reasoning or multi-step calculations. 
% By introducing CoT, the model learns to generate intermediate reasoning steps. Each step involves simpler functions that are easier for the model to learn and generalize from, compared to learning the entire complex function at once.
% Enhanced Generalization: Breaking down the reasoning process allows the model to apply learned patterns to new, unseen problems more effectively. It can reuse reasoning strategies across different tasks, improving performance.
% Error Reduction: Intermediate steps provide opportunities for error correction within the reasoning process. This reduces the likelihood of compounding errors that can occur when approximating the entire function in a single step.
% In summary, adding CoT transforms a complex function approximation task into a series of simpler tasks. This not only makes the learning process more manageable for the model but also leads to better performance on tasks that require reasoning and multi-step problem-solving.

==> ICLR/Main/2-motivations.tex <==
\vspace{-0.1in}
\section{Motivating Examples: Learning Parity Functions}
\vspace{-0.1in}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=5cm, keepaspectratio]{Figures/fig1_l4h4.pdf}
%     \caption{In this experiment, we train transformers (4 layers, 4 heads) to learn parity function with dimension $n = 30$, i.e. the entire distribution has $2^{30} \sim 10^9$ samples. To increase the hardness of the parity function, we vary $k$ from $1$ to $4$. The sample complexity is the amount of data seen by the model when it achieves perfect validation accuracy at the first time.  \jz{Define sample complexity:e.g. achieve 0.99 val accuracy;} \hz{Add Sparsity Figures; k=3, entropy vs sample complexity}}
%     \label{fig: motivating example}
% \end{figure}
% \begin{figure}[t]
%     \begin{minipage}[t]{0.45\textwidth}  % 第一张图片
%         \centering
%         \begin{subfigure}[t]{\linewidth}
%             \centering
%             \includegraphics[height=4.3cm, keepaspectratio]{Figures/fig1_l4h4.pdf}
%             \caption{}
%             \label{fig: motivating example (a)}
%         \end{subfigure}
%     \end{minipage}
%     % \hspace{0.03\textwidth}  % 调整图片之间的水平间距
%     \begin{minipage}[t]{0.45\textwidth}  % 第二张图片
%         \centering
%         \begin{subfigure}[t]{\linewidth}
%             \centering
%             \includegraphics[height=4.3cm, keepaspectratio]{Figures/fig1_plotentropy.pdf}
%             \caption{}
%             \label{fig: motivating example (b)}
%         \end{subfigure}
%     \end{minipage}
    

%     % 添加整体的图标题
%     % \captionsetup{justification=centering}  % 设置大标题的样式
%     \caption{(a) The sample complexity of training transformers (4 layers, 4 heads) to learn parity function with dimension $n = 30$. To increase the hardness of the parity function, we vary $k$ from $1$ to $4$. The sample complexity is the amount of data seen by the model when it achieves perfect evaluation accuracy at the first time.  (b) The normalized attention entropy (as defined in (\ref{eq: normalized attention entropy})) curve for the four heads of the first layer when learning $(n=30, k=3)$ parity problem. As the evaluation accuracy approaches $1$, the normalized attention entropy rapidly decreases to a low level. \huaqing{TODO: Adjust the format. Add accuracy curve. On k=3. }}
%     \label{fig: motivating example}
% \end{figure}

\begin{figure}[t]
\vspace{-0.5in}
    \centering
    \includegraphics[width=\linewidth]{ICLR/Figures/Combine_1.5.pdf}
    \caption{(a) We show that, without Chain-of-Thought (CoT), the sample complexity for training transformers to learn the parity function grows exponentially with the hardness parameter $k$. In contrast, utilizing CoT significantly improves sample efficiency.  (b) We also show that the sparsity of attention layers, measured by normalized entropy (\ref{eq: normalized attention entropy}), is crucial in the parity learning experiment. In both CoT and non-CoT scenarios, as the attention layers become sparser—indicated by a rapid decrease in normalized entropy—a corresponding jump in evaluation accuracy occurs. }
    % Here, the sample complexity is measured as the amount of data seen when the first time a model achieves perfect evaluation accuracy. 
    \label{fig: motivating example}
\vspace{-0.2in}
\end{figure}


% \caption{(a) We show the sample complexity of training transformers (4 layers, 4 heads) to learn parity function with dimension $n = 30$. We observe that the sample complexity is growing exponentially without CoT when the hardness of the problem increases, from $k =1$ to $4$. In contrast, with CoT, the training is much more sample efficient.  (b) The normalized attention entropy (as defined in (\ref{eq: normalized attention entropy})) curve for the heads of the first layer when learning $(n=30, k=3)$ parity problem. Before the evaluation accuracy approaches $1$, the normalized attention entropy rapidly decreases to a low level.}


We start with empirically exploring the sample efficiency of training transformers to learn the class of parity functions \citep{blum2003} with and without CoT. The parity functions exhibits simple structure but yet hard to learn by traditional networks \cite{abbe2018provable, malach2022hardness}. Specifically, given a set of \(n\) binary variables \(b_1, b_2, \dots, b_n\), a parity function takes $k$ secret variables \( b_{i_1}, \dots b_{i_k} \) and outputs~$1$ if the sum of these $k$ variables is odd, and $0$ if it is even:
\[ 
f(b_1, ... , b_n) = b_{i_1} \oplus b_{i_2} \oplus \cdots \oplus b_{i_k},      
\]
where $b_i \in \{0,1\}$ and $\oplus$ is the XOR operator.
For example, $f(b_1, b_2, b_3, b_4, b_5) = b_1 \oplus b_{2} \oplus b_{4} $ is a $5$-variable parity function with $k=3$. The function \(f\) returns 1 if the sum of \(b_1\), \(b_{2}\) and \(b_{4}\) is odd, and $0$ otherwise, independently of the value of $b_3$ and $b_5$. Intuitively, the parameter $k$ controls the hardness of the problem. When \(k\) increases, the number of possible subsets grows exponentially, making the identification of the correct secret set more challenging. 

Given a $n$-variable parity function~$f$, we generate sequences of length $n+2$ as auto-regressive manner: $b_1, \cdots b_{n}, b_{n+1}:=0$ and $b_{n+2}=f(b_{[1:n]})$. To incorporate CoT, we break the sum of XOR down into $k$ steps and add all the intermediate steps into the sequence, i.e. including  $b_{i_1}$, $b_{i_1} \oplus b_{i_2}$, $\cdots$, $b_{i_1} \oplus b_{i_2} \oplus \cdots \oplus b_{i_k}$. As a result, the CoT data has length $n+k+1$. 
With the example function $f(b_1, b_2, b_3, b_4, b_5) = b_1 \oplus b_{2} \oplus b_{4} $, one sampled sequence would be  
\begin{align*}
\text{No CoT } \quad & \underbrace{0, 1, 0, 1, 0}_{\mathrm{input}}, \underbrace{0}_{\mathrm{[EOS]}}, \underbrace{0}_{\mathrm{answer}} \in \{0,1\}^7, \text{ as } b_1 \oplus b_{2} \oplus b_{4} = 0 \oplus 1 \oplus 1 = 0. \\
\text{With CoT } \quad & \underbrace{0, 1, 0, 1, 0}_{\mathrm{input}}, \underbrace{0}_{\mathrm{[EOS]}} \underbrace{0, 1}_{\mathrm{CoT}}, \underbrace{0}_{\mathrm{answer}} \in \{0,1\}^{9}, \text{as } b_1 = 0, b_1 \oplus b_{2} = 1. 
\end{align*}
% \[ \underbrace{0, 1, 0, 1, 0}_{query}, 0 \in \{0,1\}^6, \text{ as } f(0,1,0,1,0) = 0 \oplus 1 \oplus 1 = 0. \] 
% , where the first $n$ tokens are independent Rademacher variables and the last token is the corresponding value of $f$. Since the last token depends on $k$-of the previous tokens, the generated sequence has an intrinsic sequential dependency of degree~$k$. 

% Under the same example, the sequence \emph{with CoT} would look like 
% \[ \underbrace{0, 1, 0, 1, 0}_{query}, \underbrace{0, 1}_{CoT}, 0 \in \{0,1\}^{8} \]  where the last three tokens are computed by $b_1$, $b_1 \oplus b_{2}$ and $b_1 \oplus b_{2} \oplus b_{4}$. 

% With the introduction of CoT, we incrementally inject the hidden steps, adding one at a time. In this case, the last three digits has sparser sequential dependency: it depends on the previous token and one hidden token, respectively $b_1, b_{2}, b_{4}$. Hence we say the sequential dependency of the CoT sequence has degree $1$. \emph{In this sense, we say CoT enables sparse sequential dependence. }

Next, we train transformer networks with and without CoT respectively, with a common held-out test set, and compare their sample complexities. The sample complexity is defined as the amount of data a model sees at the first time it achieves perfect validation accuracy. More precisely, we halt the training process when the model reaches 100\% validation accuracy and record the total number of training examples used up to this point as the empirical sample complexity.
% at training time, the model is presented with batches of training data and optimized iteratively. 

% A natural question arises: 
    % {\it How does the sample complexity scale with and without CoT, as the parity function becomes more complex?}

% \jz{Transition}
In Figure~\ref{fig: motivating example}, we compare the empirical results of learning parity function with and without CoT. The results show that the sample complexity without CoT (orange curve) grows exponentially, while with CoT (blue curve), it increases linearly. In other words, incorporating CoT allows us to learn the task with exponentially fewer samples. Additionally, it suggests that sparsity in the attention layers plays a crucial role in the learning process. To explore why CoT enables transformers to learn more efficiently, we formally define our problem setup below.

% This example also shows that expressiveness is not the bottleneck for learning parities.


 


==> ICLR/Main/acknowledgements.tex <==
\section*{Acknowledgements}
Jingzhao Zhang is supported by National Key R\&D Program of China 2024YFA1015800 and Shanghai Qi Zhi Institute Innovation Program.

==> ICLR/Main/experiments.tex <==
\begin{figure}[t]
\vspace{-0.5in}
    \centering
    \includegraphics[width=0.95\linewidth]{ICLR/Figures/Combine_Fig12.pdf}
    \caption{The sample complexity for learning parity without CoT increases exponentially with $k$. CoT significantly reduces the sample complexity, demonstrating exponential improvement across varying numbers of heads and layers.}
    \label{fig: sample complexity}
\vspace{-0.3in}
\end{figure}


\section{Empirical Experiments}\label{sec:exp}
\vspace{-0.1cm}


% \begin{figure}[t]
%     \centering
%     % 第一行 - 第一张图片
%     \begin{minipage}[t]{\linewidth}  % 设置为整行宽度
%         \centering
%         \begin{subfigure}[t]{\linewidth}
%             \centering
%             \includegraphics[width=\linewidth, keepaspectratio]{Figures/fig2.pdf}
%             \caption{}
%             \label{fig: sample complexity (a)}
%         \end{subfigure}
%     \end{minipage}

%     \vspace{0.5cm}  % 设置第一行和第二行之间的垂直间距

%         % 第二行 - 并排三张图片
%     \begin{minipage}[t]{0.30\textwidth}  % 第一张图片
%         \centering
%         \begin{subfigure}[t]{\linewidth}
%             \centering
%             \includegraphics[height=4.3cm, keepaspectratio]{Figures/fig1.pdf}
%             \caption{}
%             \label{fig: sample complexity (b)}
%         \end{subfigure}
%     \end{minipage}
%     \hspace{0.03\textwidth}  % 调整图片之间的水平间距
%     \begin{minipage}[t]{0.30\textwidth}  % 第二张图片
%         \centering
%         \begin{subfigure}[t]{\linewidth}
%             \centering
%             \includegraphics[height=4.3cm, keepaspectratio]{Figures/fig1_l4h4.pdf}
%             \caption{}
%             \label{fig: sample complexity (c)}
%         \end{subfigure}
%     \end{minipage}
%     \hspace{0.03\textwidth}  % 调整图片之间的水平间距
%     \begin{minipage}[t]{0.30\textwidth}  % 第三张图片
%         \centering
%         \begin{subfigure}[t]{\linewidth}
%             \centering
%             \includegraphics[height=4.3cm, keepaspectratio]{Figures/fig1.5.pdf}
%             \caption{}
%             \label{fig: sample complexity (d)}
%         \end{subfigure}
%     \end{minipage}
    

%     % 添加整体的图标题
%     % \captionsetup{justification=centering}  % 设置大标题的样式
%     \caption{(a), (b), (c) The sample complexity of transformers on parity problem with $n=30$ and $k=1,2,3,4$. The number of layers and heads are varied from $1$ to $4$.  (d) The sample complexity of $1$-layer $1$-head transformers with CoT on parity problem with $n=100$. \jz{without CoT uses $ > 10^9$ samples} }
%     \label{fig: sample complexity}
% \end{figure}



% In this section, we validate and extend our theoretical findings through comprehensive experiments in the following three aspects: First, we empirically confirm that CoT reduces the sample complexity in learning the parity problem for transformers with varying depths and number of heads. Second, to complement the established lower bound of sample complexity for learning parity without CoT with one-pass training, we conduct multi-pass training of transformers without CoT. The results indicate that multi-pass training indeed improves the models's ability to learn parity problems. \huaqing {But we don't claim that CoT is still much better than CoT in multi-pass case?} Third, we conduct experiments on more complex data distribution, including a synthetic data distribution representing arbitrary boolean circuits with NAND gates, and the real-world GSM8K dataset \citep{cobbe2021training}.
% \huaqing{Since we're using Adam, maybe we shouldn't use "one-pass SGD".} Although necessary simplifications are made in Section \huaqing{TODO}, in this section, the transformer architecture follows the GPT-2 architecture \citep{radford2019language} with trainable position embeddings unless otherwise specified.

In this section, we validate and extend our theoretical findings through comprehensive experiments in the following three aspects: First, we empirically confirm that CoT reduces the sample complexity of transformers in learning the parity problem. 
%with varying depths and number of heads. 
%Second, to complement the established lower bound of sample complexity for learning parity without CoT with one-pass training, we conduct multi-pass training of transformers without CoT. The results indicate that multi-pass training indeed improves the models' ability to learn parity problems. 
Second, we conduct multi-pass training of transformers without CoT, as a complement to the established lower bound (Theorem \ref{thm:nocot}) which only applies to constant-pass training. The results indicate that multi-pass training indeed improves the models' ability to learn parity problems. 
Third, we conduct experiments on the GSM8K dataset \citep{cobbe2021training} to show that CoT introduces sparse sequential dependence on real-world training data.
Although necessary simplifications on transformer are made in Section \ref{sec: theory} to develop theoretical results, we use the standard transformer architecture in the subsequent experiments following the GPT-2 architecture \citep{radford2019language} with trainable position embeddings unless otherwise specified.
\vspace{-0.1in}

\subsection {Parity Learning with Multi-layer Transformers}\label{sec: exp multi-layer}
\vspace{-0.1in}


In this section, we conduct an ablation study on the sample complexity of transformers with standard GPT-2 architectures and one-pass training,  with and without CoT.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figures/fig3_onepass.pdf}
%     \caption{The attention pattern of a $1$-layer $1$-head transformer trained on parity problem with $n=40$ and $k=20$ on a random input. The $i$-th row represents the amount that the $i$-th token attends to previous tokens. All indices $j$ for which $\mathbf s_j=1$ are marked in red. The attentions of the input tokens are not presented.\huaqing{TODO: check the notation.}%\huaqing{Should we include the conclusions in the titles, or we just discuss in the result part?}
%     }
%     \label{fig: attention pattern}
% \end{figure}




% \huaqing{Maybe we should mention that $S[i]$ here follows ascending order.}\jz{Recall $S[i]$ def when you first use it .}



\textbf{Ablation study on sample complexity~(Figure \ref{fig: sample complexity}).}
% In Figure \ref{fig: sample complexity} and \ref{fig: sample complexity with CoT and attention}a, 
%  
% In Figure \ref{fig: sample complexity}, 
We train transformers on parity problem with $n=30$ and $k=1,2,3,4$, with and without CoT, varying layers and heads from $1$ to $4$.  We choose the best performer across learning rates from $6 \times 10^{-5}$, $8 \times 10^{-5}$, and $1 \times 10^{-4}$.
At each step, a fresh batch of training data is sampled, with a maximum budget of $10^7$ samples. We record the number of samples seen by the model before reaching an evaluation accuracy of $1$ as the sample complexity. 



% Recall that sample complexity refers to the minimum number of
% samples seen by the model before reaching an evaluation accuracy of $1$.  
% In Figure \ref{fig: sample complexity}, we train transformers on the parity problem with $n=30$ and $k=1,2,3,4$, with and without CoT, varying layers and heads from $1$ to $4$.  We choose the best learning rates from $6 \times 10^{-5}$, $8 \times 10^{-5}$, and $1 \times 10^{-4}$.
% At each step, a fresh batch of training data is sampled, with a maximum budget of $10^7$ samples. Figure \ref{fig: sample complexity with CoT and attention}a shows the sample complexity of a $1$-layer $1$-head transformer on larger parity problems ($n=100$ and $20\leq k \leq 100$). Training without CoT exceeds the sample budget, so results are not shown. 
% Figure \ref{fig: sample complexity with CoT and attention}b depicts the attention pattern of a $1$-layer $1$-head transformer trained on $(n=40, k=20)$ parity problem with CoT on a random query. The CoT here processes secret variables in an ascending order. The $i$-th row represents the amount that the $i$-th token attends to previous tokens. Indices corresponding to secret variables are marked in red. The attention of the query tokens is omitted.



\begin{figure}[t]
\vspace{-0.5in}
    \centering
\includegraphics[width = \linewidth]{ICLR/Figures/Combine_fig23.pdf}
    \caption{(a) When $n$ is fixed, the sample complexity of learning parity with CoT grows approximately linearly with $k$. (b) The attention pattern learned by the transformer with CoT is \textbf{interpretable}, as the $i$-th output token of CoT predominantly attends to secret index $S[i]$.}
    % , while its attention to other tokens remains minimal.
    \label{fig: sample complexity with CoT and attention}
\vspace{-0.25in}
\end{figure}


\textbf{Results.} Figure \ref{fig: sample complexity} shows that training with CoT [first row in Figure \ref{fig: sample complexity} (a)] consistently achieves better sample efficiency than training without CoT [second row in Figure \ref{fig: sample complexity} (a)]. Moreover, for a fixed configuration of heads and layers, the sample complexity without CoT grows exponentially with the parameter $k$. In contrast, CoT greatly reduces the sample complexity, showing an exponential improvement across different numbers of heads and layers. These findings are consistent with our theoretical analysis.


\textbf{Training with CoT induce sparse and interpretable attentions (Figure \ref{fig: sample complexity with CoT and attention}).}~~We evaluate the sample complexity of a $1$-layer, $1$-head transformer on larger parity problems ($n=100$ and $20 \leq k \leq 100$). Without CoT, training exceeds the sample budget when $k \geq 4$. However, with CoT, we can successfully train for any $k$. Figure \ref{fig: sample complexity with CoT and attention}b shows the attention pattern of a $1$-layer, $1$-head transformer trained on a parity problem with $(n=40, k=20)$ using CoT on a random query. In this case, CoT processes the secret variables in ascending order. The $i$-th row illustrates the attention weight of the $i$-th token attending to the previous ones, with indices corresponding to secret variables highlighted in red. 
% Attention from query tokens is omitted for clarity.

% We show the sample complexity of a $1$-layer $1$-head transformer on larger parity problems ($n=100$ and $20\leq k \leq 100$). Training without CoT exceeds the sample budget when $k> 4$, but with CoT we are able to train for any $k$. Figure \ref{fig: sample complexity with CoT and attention}b depicts the attention pattern of a $1$-layer $1$-head transformer trained on $(n=40, k=20)$ parity problem with CoT on a random query. The CoT here processes secret variables in an ascending order. The $i$-th row represents the amount that the $i$-th token attends to previous tokens. Indices corresponding to secret variables are marked in red. The attention of the query tokens is omitted.

\textbf{Results.} In Figure \ref{fig: sample complexity with CoT and attention}a, we show that training with CoT succeed with large $n$ and $k$. Moreover, the empirical result suggests that the sample complexity of learning parity with CoT grows approximately linearly with $k$. This shows a clear contrast to without CoT setting where the required samples explodes exponentially. To validate our theorem on learning the sparse dependence, we show in Figure \ref{fig: sample complexity with CoT and attention}b that the attention pattern learned by the transformer with CoT is interpretable. Specifically, the $i$-th output token of CoT primarily focuses on the $i$-th secret variable, with minimal attention given to other tokens.  % \huaqing{TODO: More results are presented in Appendix xx.}


\begin{figure}[t]
\vspace{-0.5in}
\setlength{\abovecaptionskip}{-1pt}
    \centering
    \includegraphics[width=0.9\linewidth]{M3L/Figures/fig5_CoT.pdf}
    \caption{Evaluation accuracy of transformers on the $(n=20, k=6)$ parity problem \textbf{without} CoT. The model is trained on a dataset of $10,000$ samples for $1,000$ epochs. Almost all layer-head configuration achieve perfect evaluation accuracy. Adding more heads is more effective than adding layers. The blue dashed line marks the \textbf{with} CoT setup, which achieves perfect accuracy in 5 epochs.}
    \label{fig: multi-pass helps}
\vspace{-0.2in}
\end{figure}


\vspace{-0.1in}
\subsection{Multi-pass Training Improves Parity Learning without CoT}\label{sec:multipass}

% As suggested by our lower bound in~\Cref{thm:nocot}, analyzing the sample complexity of learning parity with multi-pass training is challenging.
%due to the correlation introduced in the gradient estimator. 
% To the best of our knowledge, there are currently no established lower bounds for the sample complexity of learning parity problems beyond constant pass training. 
% To complement the established lower bounds for transformers learning parity (\Cref{thm:nocot}), we conduct empirical experiments by training transformers \textbf{without CoT} using \textbf{multi-pass training}. The results demonstrate that multi-pass training can indeed enhance the sample efficiency of transformers. We empirically discover that the key ingredient to successfully learning the parity problem is to develop sparse attention towards previous tokens (Figure \ref{fig: repeated-data better} Right), which is similar to the role of CoT data.

In our theory, we only establish lower bounds for the sample complexity of learning parity problems with constant pass SGD training. To complement the established lower bounds for transformers learning parity (\Cref{thm:nocot}), we conduct empirical experiments by training transformers {without CoT} using \textbf{multi-pass training}. We make two observations below.
First, the results demonstrate that training with repeated data can help Transformers learn the parity function, although this process still consumes significantly more computation (epochs) than trained on CoT data  (\Cref{fig: multi-pass helps}). Second, a key difference between one-pass and multi-pass training is the development of \textbf{sparse attention} (see Figure \ref{fig: repeated-data better} Right), similar to the role of CoT shown in the previous section. This shows that the development of sparse attention is crucial even in when training without CoT on the parity data.
% \huaqing{But to theoretically characterize the improvement on sample complexity (e.g. polynomial or quasi-exponential?) needs future work.}
% \huaqing{Definition of Attention Entropy, why it can measure attention sparsity}

\textbf{Experiment protocols.} On $(n=20,k=6)$ parity problem, we conduct multi-pass training without CoT. In Figure \ref{fig: multi-pass helps}, the models are trained with $10^4$ samples for $1000$ epochs, with the number of layers and heads ranging from $1$ to $4$. In Figure \ref{fig: repeated-data better}, we compare the training of $4$-layer $4$-head transformer on $5\cdot 10^4$ and $10^6$ samples respectively. The learning rate is initialized $10^{-4}$. 
% for a \textbf{fixed number of iteration steps}. 

\textbf{Normalized attention entropy.} To measure attention sparsity, we introduce the concept of \emph{normalized attention entropy} for each attention head (illustrated in~\Cref{fig: repeated-data better} Right). Let $\mathcal{P}^{\ell,h}(\mathbf{x})[i]$ denote the attention score distribution produced by the $h$-th head in the $\ell$-th layer at the $i$-th token of input $\mathbf{x}$. The {normalized attention entropy} for the input $\mathbf{x}$ is then defined as:
\begin{align}\label{eq: normalized attention entropy} \mathrm{Ent}(\mathbf{x}; \ell, h) = \min_{i\geq 2} \frac{H(\mathcal{P}^{\ell,h}(\mathbf{x})[i])}{\log i} \in [0,1], \end{align}
where $H(\mathcal{P}) = -\int \log(\mathcal{P}) d\mathcal{P}$ is the entropy of distribution $\mathcal{P}$. The normalization term $\log i$ represents the entropy of a uniform distribution over $i$ tokens, account for the varying context length. The minimum is taken over different tokens in $\mathbf{x}$ since attention heads may specialize in extracting information for specific tokens. As a result, a lower normalized attention entropy indicates a sparser attention pattern. To compute the normalized attention entropy for each head, we would average the normalized entropy across all question-answer pairs in the validation set.


% is to account for the varying context length, where at the $i$-th token, the attention acts on the first $i$ positions. This term

% information may be transferred between layers. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{ICLR/Figures/Combine_fig67.pdf}
%     % \caption{Repeated data is better than fresh data. Left: Overfitting. Middel: Success. Right: Fail to learn.}
%     % \caption{\huaqing{TODO} Training curves of a $4$-layer $4$-head transformer on the $(n=20, k=6)$ parity problem without CoT. The model is trained with different numbers of training samples ($5000,\ 50000,\ 1000000$) while \textbf{the number of iterations is fixed}. When the number of training samples is too small, the model \textbf{overfits} the training data (a, Left). Somewhat surprisingly, when trained on a relatively small number of training samples, the model \textbf{achieves perfect evaluation accuracy} (a, Middle); However, when trained on a large number of training samples that cover most possible inputs, the model \textbf{fails to fit the training data} and achieve non-trivial evaluation accuracy (a, Right).
%     %Normalized attention entropy curve of a $4$-layer $4$-head transformer training on the $(n=20, k=6)$ parity problem without CoT. When  Each line in the graph represents the attention entropy for a head of a certain layer.
%     %When trained on a dataset of $50000$ training samples, the normalized attention entropy significantly decreases, reaching a low level as the model's accuracy approaches $1$, indicating a sparse attention mechanism.  Conversely, When trained on a dataset of $1000000$ training samples, the normalized attention entropy remains elevated.
%     %}
%     \caption{A $4$-layer $4$-head transformer is trained on the $(n=20, k=6)$ parity problem without CoT using multi-pass training. The model is trained with varying numbers of samples ($5000$, $50000$, $1000000$) and \textbf{a fixed number of training iterations}. (a) presents the loss and accuracy curves and (b) shows the normalized present entropy as defined in \huaqing{TODO}. When the number of training samples is too small, the model \textbf{overfits} the training data (a, Left). With a moderate number of training samples, the model \textbf{achieves perfect evaluation accuracy} (a, Middle), accompanied by a significant decrease in normalized attention entropy (b, Top), indicating a sparse attention mechanism. When trained on a large training set that covers most possible inputs, the model \textbf{fails to fit the training data} and to achieve non-trivial evaluation accuracy (a, Right), and the normalized attention entropy remains elevated (b, Bottom). } 
%     \label{fig: repeated-data better}
    
% \end{figure}

% \begin{figure}[t]
%     \centering
%     % 第一行 - 第一张图片
%     \begin{minipage}[t]{\linewidth}  % 设置为整行宽度
%         \centering
%         \begin{subfigure}[t]{\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{Figures/fig6.pdf}
%             \caption{Training curves of $4$-layer $4$-head transformer learning parity without CoT.}
%             \label{fig: repeated-data better (a)}
%         \end{subfigure}
%     \end{minipage}
%     \begin{minipage}[t]{\linewidth}  % 设置为整行宽度
%         \centering
%         \begin{subfigure}[t]{\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{Figures/fig7.pdf}
%             \caption{The normalized attention entropy (as defined in (\ref{eq: normalized attention entropy})) of $4$-layer $4$-head transformer learning parity without CoT on varying numbers of training samples. Each line in the graph represents the attention entropy for a head.}
%             \label{fig: repeated-data better (b)}
%         \end{subfigure}
%     \end{minipage}
%     % 添加整体的图标题
%     % \captionsetup{justification=centering}  % 设置大标题的样式
%     \caption{The transformer is trained on the $(n=20, k=6)$ parity problem without CoT using multi-pass training, detailed in ~\Cref{sec:multipass}. When the number of training samples is too small, the model \text{overfits} (a, Left). With additional samples, the model \text{achieves perfect evaluation accuracy} (a, Middle), accompanied by a significant decrease in entropy (b, Top). Surprisingly, when trained on a even larger training set, the model \text{fails to learn} (a, Right), and the normalized attention entropy remains elevated (b, Bottom).} 
%     \label{fig: repeated-data better}
% \end{figure}



% Note: no generalization gap. normalized attention indicating learns sparse attention. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/fig7.pdf}
%     \caption{Normalized attention entropy curve of a $4$-layer $4$-head transformer training on the $(n=20, k=6)$ parity problem without CoT. When  Each line in the graph represents the attention entropy for a head of a certain layer.
%     When trained on a dataset of $50000$ training samples, the normalized attention entropy significantly decreases, reaching a low level as the model's accuracy approaches $1$, indicating a sparse attention mechanism.  Conversely, When trained on a dataset of $1000000$ training samples, the normalized attention entropy remains elevated.
%     }
%      %The model is trained with different numbers of training samples ($50000,\ 1000000$) while \textbf{the number of iterations is fixed}. 
%     \label{fig: repeated data better - entropy}
% \end{figure}


\begin{figure}[t]
\vspace{-0.5in}
    \centering
\includegraphics[width=\linewidth]{ICLR/Figures/Combine_fig67.pdf}
% \vspace{-0.1in}
    \caption{$4$-layer $4$-head transformer trained on the $(n=20, k=6)$ parity problem without CoT using multi-pass training, detailed in~\Cref{sec:multipass}. When trained on a small dataset of $50000$ samples, the model \text{achieves perfect evaluation accuracy} (Top), accompanied by a significant decrease in entropy. Surprisingly, when trained on an even larger training set with $1000000$ samples, the model \text{fails to learn} (Bottom), and both the training loss and the normalized attention entropy remain elevated. This shows that the development of attention sparsity may improve optimization.}
    \label{fig: repeated-data better}
\vspace{-0.2in}
\end{figure}

\textbf{Results.} As shown in Figure \ref{fig: multi-pass helps}, when trained on $10^4$ samples, which only accounts for a small portion ($\sim 1\%$) of all possible inputs ($2^{20}\approx 10^6$), most of the transformer architectures we examined achieve perfect evaluation accuracy given sufficient epochs. While the $k=6$ problem is intractable with one-pass training without CoT, these results demonstrate that multi-pass training can indeed enhance learning in the no-CoT setup. However, CoT is by far the most effective accelerator, achieving perfect accuracy in just 5 epochs, significantly outperforming the multi-pass no-CoT training.  %and find solutions with sparse attention patterns. 
% \huaqing{Strong bias to sparse dependency?}

Although learning without CoT is less efficient, it offers a "slow-mode" trajectory. In Figure \ref{fig: repeated-data better} (Top), the no-CoT loss function initially plateaus before eventually dropping to zero. During this plateau, the entropy in the attention layers continues to decrease, indicating that feature learning is occurring gradually. When all the attention heads become sparse, a transition phase occurs in the loss and accuracy: the loss drops to zero, and evaluation accuracy jumps to 1. In contrast, in the failure case shown in Figure \ref{fig: repeated-data better} (Bottom), the entropy of the attention layers remains high throughout.

% Interestingly, with a fixed number of iterations, a model trained on a smaller dataset over more epochs achieves perfect evaluation accuracy (Figure \ref{fig: repeated-data better}, Up), while a model trained on a larger dataset with fewer epochs does not (Figure \ref{fig: repeated-data better}, Down). This contradicts the common belief that a more diverse dataset enhances models' generalization and highlights the necessity of multi-pass training for learning the parity problem without CoT. 
This experiment on no-CoT confirms that sparse attention is crucial for parity learning. As previously demonstrated in Figure \ref{fig: motivating example}, CoT accelerates learning by quickly inducing sparsity. This suggests that CoT not only improves the sample efficiency but also improve the optimization landscape by facilitating sparsity, due to the introduction of sparse dependencies added in the intermediate steps.
% As demonstrated in Figure \ref{fig: repeated-data better} Right, successful learning with a smaller dataset coincides with a significant decrease in attention entropy, indicating the development of sparse attention. In contrast, entropy remains elevated when trained on a larger dataset.
\vspace{-0.1in}
\subsection{CoT Induces Sparsity on Real-World Data}\label{sec: GSM8K}
\vspace{-0.1in}
% In previous sections, we theoretically and empirically demonstrate that CoT exponentially reduces the sample complexity required for transformers to learn the synthetic parity problem by reducing the sequential dependence. Furthermore, models trained on CoT data exhibit sparse attention patterns. In this section, we conduct experiments with pre-trained models on the real-world
Now we move from the synthetic parity problem to real world experiment on GSM8K dataset of grade-school math word problems \citep{cobbe2021training}. We observe that: 
\vspace{-0.1in}
\begin{enumerate}[leftmargin=*]
    \item Real-world CoT data also exhibits sparse sequential dependence, leading to a sparser attention pattern in pre-trained models.
    \item Fine-tuning on CoT data further enhances the models' attention sparsity on the input data.
\end{enumerate}
\vspace{-0.1in}


% As shown in Figure \ref{fig: GSM8K data}, the attention entropy i% s significantly lower for the CoT data, indicating that real-world CoT data indeed exhibits a sparser structure.
\textbf{Experiment protocols.} In Figure \ref{fig: GSM8K data}, we examine two data types: \texttt{With CoT}, where inputs from GSM8K dataset are concatenated with ground truth answers that include multiple reasoning steps, and \texttt{No CoT}, where inputs are directly concatenated with the final answer. We evaluate two language models: the pre-trained model Qwen2-7B \citep{yang2024qwen2} and the specialized mathematics model Qwen2-7B-Math \citep{qwen2024} which is fine-tuned from Qwen2-7B on a mathematics-specific corpus with CoT data. 
We plot the normalized attention entropy (\Cref{eq: normalized attention entropy}) across different heads. More details can be found in the Appendix \Cref{sec: experiment detail}. % \huaqing{TODO. normalized attention entropy. data format, average over test set. Model architecture (28 heads and layers)}.

\textbf{Results.}
Unlike the synthetic parity problem, the sequential dependency of real-world data is hard to measure directly. However, it can be inferred from the attention sparsity of pre-trained models when they process such data as input. As shown in Figure \ref{fig: GSM8K data}, comparing the normalized attention entropy of the same pre-trained model Qwen2-7B on different types of data, we can see that the entropy is lower for \texttt{With CoT} data compared to \texttt{No CoT} data, indicating that real-world CoT data indeed exhibits a sparser structure. Furthermore, on the same \texttt{With CoT} data, Qwen2-Math-7B model demonstrates lower attention entropy compared to Qwen2-7B model, suggesting that fine-tuning on CoT data promotes the development of sparser attention patterns in the model.

% We then evaluate the attention sparsity of two language models, Qwen2-7B and Qwen2-Math-7B \huaqing{cite}, using the GSM8K dataset. Qwen2-Math-7B is a specialized mathematics language model developed from Qwen2-7B and fine-tuned on a mathematics-specific corpus. As illustrated in Figure \ref{fig: GSM8K model}, Qwen2-Math-7B demonstrates sparser attention compared to Qwen2-7B when processing the same input, suggesting that fine-tuning on Chain-of-Thought (CoT) data promotes the development of sparser attention patterns in the model.%which contains 

% In the parity problem we consider above, CoT clearly reduces the dependency degree from $k$ to $1$. However, the dependency degree of real-world data is hard to measure directly. Thus 

% We use the GSM8K dataset \citep{cobbe2021training}


% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figures/fig_GSM8K_ex1.pdf}
%     \caption{CoT fine-tuning makes the model's attention pattern sparse.}
%     \label{fig: GSM8K model}
% \end{figure}




==> ICLR/Main/related.tex <==

\vspace{-0.12in}
\section{Additional Related Work}
\begin{figure}[t] 
% \setlength{\abovecaptionskip}{-1pt}
\vspace{-0.5in}
    \centering
    \includegraphics[width=\linewidth]{Figures/fig_GSM8K_combine_overlap.pdf}
    \caption{We compare the normalized attention entropy of the pre-trained Qwen2-7B and math-specialized Qwen2-Math-7B models on the GSM8K dataset with and without CoT prompting (Section \ref{sec: GSM8K}). Each bar represents the entropy of an attention head. The Qwen2-7B model exhibits sparser attention when processing CoT data, indicating that real-world CoT data has a sparser structure. The entropy difference between the Qwen2-7B and Qwen2-Math-7B model suggests that fine-tuning on CoT data promotes the development of sparser attention patterns of the model.}
    \label{fig: GSM8K data}
    \vspace{-0.28in}
\end{figure}
\vspace{-0.1in}
\textbf{Parity Learning.} The most relevant work to ours is~\cite{wies2023subtask}, which shows that subtask decomposition enables learning the parity problem with polynomial sample complexity in recurrent neural networks (RNNs). Their learnability results rely on techniques from~\cite{wang2022provablegeneralizationrecurrentneural}, which operate within the NTK linearization regime of RNNs. In contrast, the Transformers analyzed in our work exhibit feature learning and identify the sparse secret set within the attention module. On the positive side, a line of works that studies optimization dynamics of neural networks on parity~\citep{kou2024matchingstatisticalquerylower,barak2023hiddenprogressdeeplearning,edelman2023paretofrontiersneuralfeature,daniely2020learningparitiesneuralnetworks,abbe2023sgdlearningneuralnetworks,abbe2024mergedstaircasepropertynecessarynearly} show that $n^{\Omega(k)}$ samples is sufficient to learn parity, which is close to the statistical query lower bound \citep{kearns1998efficient}. 
%On the negative side, it has been shown that in SGD learning with \textbf{additional noise}, $n^{\Omega(k)}$ samples are indeed needed \citep{shalevshwartz2017failuresgradientbaseddeeplearning,abbe2020polytimeuniversalitylimitationsdeep}. 
{On the negative side, it is well-established that learning parity using gradient descent (GD) requires $\Omega(n^k)$ iterations due to the SQ lower bound \citep{kearns1998efficient}. For SGD learning, \cite{shalevshwartz2017failuresgradientbaseddeeplearning,abbe2020polytimeuniversalitylimitationsdeep} showed that an exponential number of samples is necessary when SGD is hindered by additional noise or when the number of weights updated in each step is constrained. } However, it remains unclear whether standard mini-batch SGD will still need exponential sample complexity. In our paper, we take the alternative approach to consider the training as an online algorithm with bounded memory (parameters) and utilize results from online learning literature to provide a rigorous exponential lower bound \citep{lyu2023tighttimespacelowerbounds,kol2017time}. \cite{hahn2024sensitivefunctionshardtransformers} shows that while parity is easy to represent using Transformers, the sensitivity structure of the function will require the representation to have large weight norms. {A recent work \citep{abbe2024far} conjectured that a distribution is weakly learnable by a Transformer if and only if it has constant globality, which is supported by empirical experiments. The work also highlights the parity problem as a notable special case.}
 
\textbf{Chain-of-Thoughts (CoT).} CoT is the technique to let the model generate a reasoning process before final answers.
CoT prompting has proven effective in enhancing language models' reasoning capabilities~\citep{wei2022chain,zhang2022automaticchainthoughtprompting,wang2023planandsolvepromptingimprovingzeroshot,zhou2023leasttomostpromptingenablescomplex,wang2024chainofthoughtreasoningprompting,creswell2023selectioninference}. Training with CoT data has further improved the model's capability in performing complex reasoning (see~\citet{qwen2024,yue2023mammothbuildingmathgeneralist,yu2024metamathbootstrapmathematicalquestions,kim2023cotcollectionimprovingzeroshot} and reference therein).
Different lines of work have explored the effect of CoT. From the representation theory perspective, works including \cite{feng2024towards,merrill2024expressivepowertransformerschain,li2024chainthoughtempowerstransformers,nowak2024representationalcapacityneurallanguage,wen2024rnnstransformersyetkey} show that CoT can provably expand the representation power of neural architectures including Transformers and RNNs. From the statistical approximation level, prompting with CoT reduces the statistical error \citep{hu2024unveilingstatisticalfoundationschainofthought,prystawski2023thinkstepstepreasoning}. \cite{li2023dissectingchainofthoughtcompositionalityincontext} studies how MLP learns with CoT data. \cite{li2024how} studies how Transformers learn to perform CoT through prompting using gradient descent. We differ from this work as (1) we focus on how Transformer captures the sparse sequential dependency in CoT, which is not reflected in their data modeling; (2) we study zero-shot CoT data directly. \citet{dutta2024thinkstepbystepmechanisticunderstanding,wang2024understandingtransformerperformmultistep} studies pre-trained Transformers' activation on CoT data. They highlight the attention head's role in moving the essential information from the context to the reasoning process, which is consistent with our theoretical insight. Concurrently with our work, \citet{juno2024transformer} theoretically demonstrated that CoT reduces the number of gradient steps required to solve the parity problem. While their analysis focuses on GD with a noisy oracle, our work investigates mini-batch SGD and provides theoretical guarantees on the exponential reduction in sample complexity.

We defer other related works to~\Cref{sec:app:related}.

\vspace{-0.2in}
\section{Conclusion and Future Works.} 
\vspace{-0.1in}
Our work demonstrates that Transformers trained on Chain-of-Thought (CoT) data with sparse sequential dependencies can efficiently learn sparse attention mechanisms, accurately capturing these dependencies while requiring exponentially fewer samples than models trained without CoT. Our current analysis of CoT training assumes that each subsequent token depends on exactly one token in the context and focuses solely on the parity function. A promising future direction is to explore more general scenarios where each token depends on multiple previous tokens and extends to function classes beyond parity.
\newpage

==> ICLR/Main/theory.tex <==
\vspace{-0.1in}
\section{Theoretical Analysis} \label{sec: theory}
\vspace{-0.1in}
In this section, we provide a formal analysis of the training dynamics of Transformers on the parity problem, both with and without Chain of Thought (CoT). We select the parity problem as our testbed because identifying a set of key variables amidst various confounding ones is a fundamental aspect of many reasoning tasks, and parity serves as an abstraction of this process.


\vspace{-0.1in}
\subsection{Notations and Definitions}


% \textbf{Notation.} We use $\oplus$ to indicate the XOR operator on binary variables. 
% We use $e_i$ to denote the $i$-th one-hot vector and specify the dimension in the context. We will use $[j]$ to denote variables corresponding to the $j-$th token dimension without otherwise specified. We will use $p(x, y)$ to indicates $2(x - 1) + y$. 

\textbf{Parity Problem.} Each token in our setting is either $0$ or $1$. We represent a sequence of length $T$ as $\bsequence[1], \ldots, \bsequence[T]$. A parity function is a function of form $\mathrm{parity}_S (\bsequence) = \oplus_{j \in \mathcal{S}} \bsequence[j]$, where $\mathcal{S}$ is the set of secret indices that is fixed during training and testing, and $\oplus$ is the XOR operator on binary variables. The cardinal of the secret set $k = |S|$  controls the hardness of the problem. 





% \textbf{Data Distribution.} We will study language modeling on the well-known \emph{parity} problem. In our setting, every token takes the value of 0 or 1 and we will denote a sequence of binary variables with length $T$ as $\bsequence[1], \ldots, \bsequence[T]$. The parity problem requires the model to calculate the the sum of bits on a set of secret indices. We will denote the set of secret indices as $\mathcal{S}$. 


% For standard sequences without CoT, the parity of the sum of bits on the secret indices is appended at the end of the sequence directly.
\begin{definition}[Parity Problem $(n,k)$ without CoT]
\label{def:nocot}
Given a secret set $\mathcal{S}$ of cardinal $k$, we define the parity problem without CoT as the following distribution of sequences $\pdatanocot$:
    \begin{align*} 
        \bsequence[i] \sim U(\{0,1\}), \forall i \in [1,n],
        \bsequence[n + 1] = 0, 
        \bsequence[n + 2] = \mathrm{parity}_S (\bsequence).
    \end{align*}
where $\bsequence[1], ..., \bsequence[n]$ are uniformly sampled from $0$ and $1$.  
\end{definition}

\begin{definition}[Parity Problem $(n,k)$  with CoT]
\label{def:cot} Given a secret set $\mathcal{S}$ of cardinal $k$, 
    we define the parity problem with CoT as the following distribution of augmented sequences $\pdatacot$:
    \begin{align*} 
        \bsequence[i] \sim U(\{0,1\}), \forall i \in [1,n],
        \bsequence[n + 1] = 0, 
        % \bsequence[n + 1+ i] = \oplus_{j=1}^i \bsequence[S[j]], \forall i \in \{ 1 , \ldots,  k \}.
        \bsequence[i + 1] = \bsequence[i] \oplus \bsequence[S[i]], \forall i \in \{ n + 1 , \ldots,  n + k \}.
    \end{align*}
    where $S$ is any permutation of $\mathcal{S}$, i.e. $\{S[i] \mid i = n + 1 , \ldots, n + k \} = \mathcal{S}$. 
\end{definition}
When CoT is provided, the data includes a step-by-step computation of the desired parity function, adding one variable at a time. Note that CoT is not unique for a given secret set since we can arbitrarily permute $\mathcal{S}$, given the commutative property of the XOR operator.


\textbf{Transformer Architecture.} To conduct the theoretical analysis, we simplify the Transformer architecture similar to prior works (see e.g. \cite{wang2024transformersprovablylearnsparse,nichani2024transformerslearncausalstructure,pmlr-v202-li23p}). More precisely, we drop all the layer norms or batch normalization; simplify the positional embedding; use a square matrix to represent the attention layer and concatenate the residual branch in a Densenet fashion~\cite{huang2017densely}. After simplification, the network still has strong expressive power like the standard Transformers.

% The major deference is that the  attention is directly parameterized by a square matrix, and that we concatenate, instead of adding, the residual branch. We first define the embedding for a binary input sequence.

In a standard Transformer, an embedding layer matches each vocabulary token into a dense vector of size $d$ and then adds a positional embedding. In our case, we only have boolean tokens and the sequence has constant length~$T$. Hence, we simply freeze $2T$ unit vectors as the embedding vectors: 
\begin{definition}[Embedding Module]
\label{def:embed}
For any position $i \in [T]$, we sample two embedding vectors $e_{i,0}$ and $e_{i,1}$ uniformly at random from unit hypercube $\mathrm{U}\left(\{\frac{1}{\sqrt{d}}, -\frac{1}{\sqrt{d}}\}^d \right)$. These embedding vectors are frozen during training.
% a set of near orthogonal vectors with unit norm.
% \begin{align*}
%     e_{p(j, l)} \sim \mathrm{U}\left(\{\frac{1}{\sqrt{d}}, -\frac{1}{\sqrt{d}}\}^d \right).
% \end{align*}
Then for any binary sequence $\bsequence \in \{0, 1\}^T$, the embedding is   defined as 
    \begin{align*}
        \embed \left( \bsequence \right) =[e_{(i, \bsequence[i])}]_{i \in [T]} \in \R^{d \times T}.
    \end{align*}
Due to the properties of the hypercube, with high probability, the embedding vectors are near-orthogonal with each other.
\end{definition}

% \begin{definition}[Embedding Module]
% \label{def:embed}
% For any position $i \in [T]$, $l \in \{0, 1\}$, we will sample vector $e_{p(j, l)}$ is sampled uniformly at random from a set of near orthogonal vectors with unit norm.
% \begin{align*}
%     e_{p(j, l)} \sim \mathrm{U}\left(\{\frac{1}{\sqrt{d}}, -\frac{1}{\sqrt{d}}\}^d \right).
% \end{align*}
% The embedding function over a binary sequence $\bsequence \in \{0, 1\}^T$ is then defined as,
%     \begin{align*}
%         \embed \left( \bsequence \right) =[e_{p(i, \bsequence[i])}]_{i \in [T]} \in \R^{d \times T}.
%     \end{align*}
% This embedding is then fixed during training.
% \end{definition}



Next, we define the attention layer. In standard architecture, the attention layer is derived from the product of query and key matrices, i.e. $QK^T = \hiddenstate^T W^Q (W^K)^T \hiddenstate$. In our case, we directly use a full matrix $\hiddenstate^T A \hiddenstate$ to parameterize it, which has the same representation power. 
\begin{definition}[Attention Module]
\label{def:attn}
Given an input matrix $\hiddenstate \in \R^{d \times T}$ and attention weight $A$, we define the attention module as 
    \begin{align*}
        &\attention(\hiddenstate) = \hiddenstate \  \softmax(C + \hiddenstate^T\qk \hiddenstate),
    \end{align*}
    where $C \in \R^{T \times T}$ is the autoregressive mask with value $-\infty$ on the lower triangular matrix.     
    % value $0$ on the upper right triangle (including the diagonal line) and $-\infty$ at other values. The $\softmax$ is applied column-wise. 
\end{definition}

% \begin{definition}[Attention Module]
% \label{def:attn}
%     We define the attention function over a matrix $\hiddenstate \in \R^{d \times T}$ as 
%     \begin{align*}
%         &\attention(\hiddenstate) = \hiddenstate \  \softmax(C + \hiddenstate^T\qk \hiddenstate).
%     \end{align*}
%     Here $C \in \R^{T \times T}$
%     is the autoregressive mask with value $0$ on the upper right triangle (including the diagonal line) and $-\infty$ at other values.The $\softmax$ is applied column-wise. 
% \end{definition}


% Compared with standard attention, the attention module defined in~\Cref{def:attn} fixes the value matrix as identity and merges the $Q$ and $K$ matrices as there is only one head here.

The attention module is then followed by a fully connected layer with ReLU activation:
\begin{definition}
\label{def:ffn}  
 We define the FFN function with width $2m$ over a matrix $\hiddenstate \in \R^{2d \times T}$ as 
 \vspace{-1mm}
 \begin{align*}
     \FFN(\hiddenstate) = \head^T \relu( \weight X).
 \end{align*}
 \vspace{-1mm}
Here $\weight \in \R^{2m \times 2d}, \head \in \R^{2m \times o}$ with $o$ being the output dimension and $\relu$ is element-wise. 
\end{definition}

Finally, we concatenate the modules into a simplified Transformer block.
\begin{definition}[Simplified Transformer Block]
\label{def:trans}
We define a simplified Transformer block as,
\vspace{-1mm}
\begin{align*}
    \transformer(\bsequence) = \FFN\left(\begin{bmatrix} 
    \embed\left( \bsequence \right) \\
    \attention\left(\embed\left( \bsequence \right) \right) \end{bmatrix} \right),
\end{align*}
% \vspace{-1mm}
where $\embed$ is the embedding module, $\attention$ is the attention module and $\FFN$ the fully connected layer. An $L$-layer Transformer consists of a composition of $L$ such blocks, with the embedding module $\embed$ appearing only in the initial layer. The intermediate dimension is set to $d$, while the output dimension of the final layer is 1. 
\end{definition}

Compared with the standard residual structure, we use a Densenet structure to concatenate the residual branch with identity branch. Again, this transformation does not affect the representation power of the network, which is the standard practice in previous theoretical analysis (see e.g. \citet{wang2024transformersprovablylearnsparse,nichani2024transformerslearncausalstructure}).

\textbf{Loss function.} To simplify our analysis, we use hinge loss $\ell(\hat y, y) = \max\{ (-1)^y \hat y + 1, 0\}$ as the loss function. We define the next token prediction loss of a boolean sequence $\bsequence$ as  $ L(w) =   \ell( \transformer^{(L)}(\bsequence)[n+1], \bsequence[n + 2])$ and
$ L(w) =  \sum_{i = n + 1}^{n + k} \ell( \transformer^{(L)}(\bsequence)[i], \bsequence[i + 1])$ for with and without CoT setup respectively,
where $w$ denotes all the trainable parameters.% $[A, W]$ in the attention module and the FFN map across all layers. 
% Further, $T[w]$ indicates the parameterization defined in this section. In the following text, the notation $[w]$ is omitted when its meaning is clear from the context.


\subsection{Exponential Sample Complexity without CoT}

We now present analysis in the no CoT setup. First, we show that the parity problem is easy to represent with the simplified Transformer architecture:

% \begin{theorem}[Easy to Represent]
% \label{thm:rep}
%      Consider the Transformer model defined in~\Cref{def:trans}, for any $\delta < 0.1$ and large enough $n$, with probability at least $1 - \delta$ over the randomness of embedding $e$, there exists a weight configuration of the Transformer with dimension $d = \tilde \Omega(k)$ and width $2m = \Omega(k)$, such that it can achieve perfect accuracy on the parity problem $(n,k)$ without CoT, i.e.
%     \begin{align*}
%         \forall \bsequence \sim \pdatanocot, \sgn\left(\transformer(\bsequence)[n + 1] \right) = \bsequence[n + 2].
%     \end{align*}
%     % Further, when the number of secret indices $k$ is in $[n / \log^5 (n / \delta), n / \log^4(n/\delta)]$, there exists a weight configuration that can be stored in $o(nk)$ memory. \kaiyue{Change $d$ depends on $k$.}
% \end{theorem}

\begin{theorem}[Easy to Represent]
\label{thm:rep}
     % Consider the Transformer model defined in~\Cref{def:trans}, for any $\delta < 0.1$ and large enough $n$, with probability at least $1 - \delta$ over the randomness of embedding $e$, there exists a weight configuration of the Transformer with dimension $d = \tilde \Omega(k)$ and width $2m = \Omega(k)$, such that it can achieve perfect accuracy on the parity problem $(n,k)$ without CoT, i.e.
     Consider the Transformer model defined in~\Cref{def:trans}, for any $\delta<0.1$ and large enough $n$, when the number of secret indices $k$ is in $[n / \log^5 (n / \delta), n / \log^4(n/\delta)]$, with probability at least $1 - \delta$ over the randomness of embedding $e$, there exists a weight configuration of the Transformer with dimension $d = \Theta(k\log (n/\delta))$ and width $2m =O(k)$ with $\Theta(\log n)$ precision of the weights and activations, such that $d^2+dm=o(nk/\log n)$, and it achieves perfect accuracy on the parity problem $(n,k)$ without CoT, i.e.
     % \vspace{-2mm}
    \begin{align*}
        \forall \bsequence \sim \pdatanocot, \sgn\left(\transformer(\bsequence)[n + 1] \right) = (-1)^{\bsequence[n + 2]+1}.
    \end{align*}
    % \vspace{-2mm}
    % Further, when the number of secret indices $k$ is in $[n / \log^5 (n / \delta), n / \log^4(n/\delta)]$, there exists a weight configuration that can be stored in $o(nk)$ memory. \kaiyue{Change $d$ depends on $k$.}
\end{theorem}

In other words, the model possesses sufficient expressive power to represent any parity function, even in the absence of the chain of thought. Therefore, we are in the \emph{representational-sufficient} regime where expressiveness is not the bottleneck. The proof of this statement is based on random matrix theory and concentration inequalities, which we defer to~\Cref{app:thm:rep}. 
% This theorem shows that the problem we are analyzing falls in the \emph{representational-sufficient} regime, where the model has the representational power to represent solution to the reasoning problem, even without the presence of the chain of thought.

While the function is expressible, this does not guarantee that the solution can be easily found. In fact, we show that achieving a perfectly accurate solution using a gradient-based optimization method requires an exponential number of samples in $k$ assuming the memory, i.e. space complexity, to perform optimization is bounded throughout the training.


\begin{theorem}[Hard to Learn]
\label{thm:nocot}
For any randomly initialized simplified Transformer model with constant layers, when the embedding dimension $d$ and width $2m$ satisfies $d^2 + dm = o(nk / \log(n))$, for any constant number of passes $q$, when the model is trained with $q-$pass stochastic gradient descent with $O((d^2 + dm)\log n)$ memory, the sample complexity required to learn the parity problem $(n,k)$ without CoT to any nontrivial accuracy $a > 50\%$ with nontrivial probability $p > 50\%$ is $2^{\Omega(k)}$.
\end{theorem}

The proof is deferred to~\Cref{app:thm:nocot}. We use results from the classical online learning communities~\citep{lyu2023tighttimespacelowerbounds} to show that in the regime where the memory required to perform the training is less than $nk$, the model can't effectively store information about enough samples inside the parameters during training, and hence can't infer the secret indices effectively. Here the parameters $k$ denotes the size of the secret set $\mathcal{S}$ and the sample complexity grows exponentially when $k$ grows.

\subsection{Polynomial Sample Complexity with CoT}

The result in~\Cref{thm:nocot} presents a seemingly negative outcome for learning algorithmic reasoning, as the model requires exponentially many samples relative to $k$. However, in our main result,~\Cref{thm:main}, we will demonstrate that the sample complexity can be significantly reduced if a step-by-step derivation is provided. In other words, CoT is much more sample efficient, where model can effectively learn complex relationships as long as each token depends on only a few previous tokens.

% The above~\Cref{thm:nocot} seems a negative message for learning algorithmic reasoning because the model fails to learn the key variables unless exponentially many samples with respect to $k$ are provided. However, we will show that the sample complexity can be drastically reduced if a step-by-step derivation is provided in our main~\Cref{thm:main}. This suggests that the model can learn complex relationships effectively as long as each token only depends on a few previous tokens. 


We will use the following initialization of the 1-layer Transformer model. The attention is initialized to be uniform ($A = 0$) and the contribution of attention output is initialized to be zero ($W_{r, d+1:2d} = 0$). The parameter $\head$ in the FFN and the word embedding $\embed$ is fixed during training.

\begin{assumption}[Initialization]
\label{assum:init}
At initialization, 
\begin{align*}
    \forall r \in [2m], A &= 0, W_{r, d + 1: 2d} = 0, 
    W_{r, 1:d} = \sum_{i = n + 1}^{n + k} \sum_{b = 0}^1 \nu_{r, i, b} e_{i, b}, h_{1:m} = \frac{1}{2m}, h_{m+1:2m} = -\frac{1}{2m}.
\end{align*}
Here $\nu_{r, i, b}$ is independent random variable sampled uniformly from $\{-\epsilon, \epsilon\}$. 
\end{assumption}

We can then train the model with stochastic gradient descent (SGD) and get the following theorem.

\begin{theorem}[Easy to Learn with CoT]
    \label{thm:main}
    For any constant $\delta \in (0,1)$,  when the number of secret indices $k$ is in $[n / \log^5 (n / \delta), n / \log^4(n/\delta)]$, with probability $1 - \delta$, a randomly initialized simplified Transformer (see~\Cref{assum:init}) with $o(nk)$ parameters trained for constant steps using mini-batch SGD with $\Tilde O(n)$ samples using appropriate hyperparameters (see~\Cref{assum:order}) can reach perfect accuracy on a parity problem $(n,k)$ with CoT,
    \begin{align*}
        \forall \bsequence \sim \pdatacot, i \in \{n + 1, \ldots, n + k\},\sgn\left(\transformer(\bsequence)[i] \right) = \bsequence[i + 1].
    \end{align*}
    Furthermore, after training, the attention pattern is interpretable and one-hot in the sense that, for any $\bsequence \sim \pdatacot, i \in \{n + 1,\cdots,  n + k\}, j\leq i$,
    \begin{align*}
        \big| \softmax(C +  \embed(\bsequence)A\embed(\bsequence) )[j, i] - \1(j = S[i])  \big| < 1/n^8.
    \end{align*}
    Moreover, the result still holds even if all the weights and activations are  in $\Theta(\log n)$ precision.
\end{theorem}

This theorem indicates that the attention module can successfully extract the sparse sequential dependencies in the CoT data and faithfully represent it in the attention pattern, which is validated in our experiments (see \Cref{fig: sample complexity with CoT and attention}). It is also amongst the first optimization dynamics analysis of Transformers using finite-sample gradients rather than population gradients. We delay the full proof of the theorem to~\Cref{sec:proofofthm3}.

\emph{Proof Sketch.} In our analysis, the dynamics of the model includes three key phases. In the first phase, the weight of the FFN layers become correlated with the embeddings associated to the secret indices. In the second phase, this correlation caused the attention module to receive a strong signal to amplify the attention weight on the corresponding secret indices at each position. The attention pattern will become one-hot after this step. Finally, in the third phase, the FFN layers learn the correct mapping to the output, utilizing both the embedding at the current token and the retrieved embedding from the secret indices as indicated by the attention.

\textbf{Phase 1. Configuring the FFN} At initialization, as the FFN weight corresponds to the attention output ($W_{r, d+1:2d}$) is initialized to be zero. The set of neurons activated at each position $i \in [n+1, n+k]$ is solely determined by the word embedding $e_{(i,\bsequence[i])}$ at the position. Because $e_{i, b}$ are nearly orthogonal, it holds that $\langle e_{i,\mathbf b[i]},W_{r,1:d}\rangle \approx \nu_{r,i,b}$ for all $i$ and $r$ with high probability. As a result, for a fixed $i$ and $\mathbf{b}[i]$, the set of activated neurons at position $i$ is $\{r \mid \nu_{r, i, \bsequence[i]} > 0 \}$. Therefore, at initialization, the MLP can be viewed as an ensemble of multiple linear functions specialized to each position and boolean value. We can show that when the learning rate is small, the set of activated neurons at each position remains the same through the training process. Hence, we can conceptually view the FFN function as a set of different linear functions applied independently at each position and value. We will denote this set of linear weight as $\kappa_{t,i,b}$ (formally defined in~\Cref{lem:attnsignal}).

As the attention weight matrix $\qk$ is initialized as zero, the attention pattern will be uniform at initialization. Notice that in the parity data with CoT, the only position whose value correlates with $\bsequence[i + 1]$ when conditioned on $\bsequence[i]$ is $S[i]$. This suggests that the linear weight $\kappa_{1,i,\bsequence[i]}$ will have a stronger correlation with the embedding $e_{(S[i], \bsequence[j])}$ than other embeddings. 

This step crucially relies on the sparse dependency in the CoT data. The strong linear correlation will not be present in the data without CoT when $k > 1$, as every token $\bsequence[i]$ for $i \in [n+1]$ will be uncorrelated with the desired output $\bsequence[n + 2]$ in such case.


\textbf{Phase 2. Learning the Sparse Attention} 
At the second step, as  the FFN weight corresponds to the attention output is no longer zero, the attention weight matrix $\qk$ will receive a non-zero gradient. By the chain rule, the gradient corresponding to how the attention from $i-$th token attends to the $j-$th token  $\softmax(C + \hiddenstate^T\qk \hiddenstate)[j,i]$ will be larger when the approximate contribution of the embedding of the $j-$th token to the output at the $i-$th token $\langle \kappa_{1,i,\bsequence[i]}, e_{(j, \bsequence[j])} \rangle$ is larger. This suggests that the attention will be amplified on the index that has a strong correlation with the output at the current token, which is the secret index $S[i]$. This step will make the attention pattern approximately one-hot as in the theorem statement.



\textbf{Phase 3. Learning the Output Mapping} 
At the final step, as the attention pattern is one-hot, the FFN layer only needs to learn a mapping from the embedding at the current token and the embedding at the secret index to the output. As the mapping is linear conditioned on the embedding at the current token, the FFN layer can learn the correct mapping within a single step. This step will make the model reach perfect accuracy on the parity problem with CoT.


\vspace{-0.1in}




